Efficient Approximate Search for Sets of Vectors

We consider a similarity measure between two sets $A$ and $B$ of vectors, that balances the average and maximum cosine distance between pairs of vectors, one from set $A$ and one from set $B$. As a motivation for this measure, we present lineage tracking in a database. To practically realize this measure, we need an approximate search algorithm that given a set of vectors $A$ and sets of vectors $B_1,...,B_n$, the algorithm quickly locates the set $B_i$ that maximizes the similarity measure. For the case where all sets are singleton sets, essentially each is a single vector, there are known efficient approximate search algorithms, e.g., approximated versions of tree search algorithms, locality-sensitive hashing (LSH), vector quantization (VQ) and proximity graph algorithms. In this work, we present approximate search algorithms for the general case. The underlying idea in these algorithms is encoding a set of vectors via a "long" single vector. The proposed approximate approach achieves significant performance gains over an optimized, exact search on vector sets.

==> Makefile <==
# Makefile for thesis.
# Simply run `make` to build the thesis.pdf.
# You can also use `make pvc` to "preview continuously" (i.e. pdf will update
# in real time while editing the source files).
# Use `make clean` to remove all generated files.
# Note that all auxilliary files will be stored in the `aux` directory to keep
# the root directory clean.
#
# This is roughly based on: 
# https://drewsilcock.co.uk/using-make-and-latexmk
# http://tex.stackexchange.com/questions/40738/how-to-properly-make-a-latex-project
#

LATEX=xelatex
LATEXOPT=--shell-escape
NONSTOP=--interaction=nonstopmode
AUXDIR=aux

LATEXMK=latexmk
LATEXMKOPT=-pdf -outdir=$(AUXDIR) -auxdir=$(AUXDIR)
CONTINUOUS=-pvc

MAIN=thesis
OUTPUT_FILENAME=thesis
SOURCES := Makefile $(shell find . -regex '.*\.\(tex\|cls\|sty\|bib\)')
ADDITIONAL_FILES := README.md
FIGURES := $(shell find graphics/* -type f)

all: symlink once

once: symlink
	$(LATEXMK) $(LATEXMKOPT) -pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

.refresh:
	touch .refresh

pvc: aux $(MAIN).tex .refresh $(SOURCES) $(FIGURES)
	$(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) -pdflatex="$(LATEX) $(LATEXOPT) $(NONSTOP) %O %S" $(MAIN)

# Create a symlink for the final PDF
symlink: aux
	rm -f $(OUTPUT_FILENAME).pdf
	ln -Fs $(AUXDIR)/$(MAIN).pdf $(OUTPUT_FILENAME).pdf

clean:
	$(LATEXMK) -C $(MAIN) -quiet
	$(shell echo "find . -name '*.aux' -print0 | xargs -0 rm -f")
	$(shell find . -name '*.aux' -print0 | xargs -0 rm -f)
	rm -rf aux
	rm -f .refresh
	rm -f $(MAIN).pdfsync
	rm -rf *~ *.tmp
	rm -f *.bbl *.blg *.end *.fls *.log *.out *.fdb_latexmk *.cb *.thm
# not removing the biber cache - it's not guaranteed that biber is even available,
# or that biber --cache gives something meaningful

aux:
	mkdir -p aux aux/front aux/back aux/misc aux/main

$(MAIN).zip: $(SOURCES) $(FIGURES) $(ADDITIONAL_FILES)
	rm -f $(MAIN).zip
	zip $(MAIN).zip $(SOURCES) $(FIGURES) $(ADDITIONAL_FILES)

archive: $(MAIN).zip
zip: $(MAIN).zip


.PHONY: clean once symlink all aux

